Dynamic Gaussian Mixture based Deep Generative Model For Robust Forecasting on Sparse Multivariate Time Series

Forecasting on sparse multivariate time series (MTS) aims to model the predictors of future values of time series given their incomplete past, which is important for many emerging applications. However, most existing methods process MTS's individually, and do not leverage the dynamic distributions underlying the MTS's, leading to sub-optimal results when the sparsity is high. To address this challenge, we propose a novel generative model, which tracks the transition of latent clusters, instead of isolated feature representations, to achieve robust modeling. It is characterized by a newly designed dynamic Gaussian mixture distribution, which captures the dynamics of clustering structures, and is used for emitting timeseries. The generative model is parameterized by neural networks. A structured inference network is also designed for enabling inductive analysis. A gating mechanism is further introduced to dynamically tune the Gaussian mixture distributions. Extensive experimental results on a variety of real-life datasets demonstrate the effectiveness of our method.

==> Sections/introduction2.tex <==
\section{Introduction}

Multivariate time series (MTS) analysis is heavily used in a variety of applications, such as cyber-physical system monitoring \cite{zhang2019deep}, financial forecasting \cite{binkowski2018autoregressive}, traffic analysis \cite{li2018diffusion}, and clinical diagnosis \cite{che2018recurrent}. 
% \scream{Do you mean "clinical diagnosis"?} 
Recent advances in deep learning have spurred on many innovative machine learning models on MTS data, %such as autoregressive neural networks \cite{} and deep Markov models \cite{krishnan2016structured},
which have shown remarkable results on a number of fundamental tasks, including forecasting \cite{qin2017dual}, event prediction \cite{choi2016retain}, and anomaly detection \cite{zhang2019deep}. Despite these successes, most  existing models regard the input MTS as homogeneous and complete sequences. In many emerging applications, however, MTS signals are integrated from heterogeneous sources and are very sparse.

\begin{figure}[!t]
\includegraphics[width=1.0\columnwidth]{Figures/fig_intro.pdf}
\caption{An illustration of latent structures underlying the sparse MTS of two dialysis patients. The vector below each state is a temporal feature generated from some distribution.}\label{fig.intro}
\vspace{-0.3cm}
\end{figure}

For example, consider MTS signals collected for dialysis patients. Dialysis is an important renal replacement therapy 
for purifying the blood of patients whose kidneys are not working normally \cite{inaguma2019prediction}. Dialysis patients usually have routines of dialysis, blood tests, chest X-ray, etc., %meanwhile are
which record data such as venous pressure, glucose level, and cardiothoracic ratio (CTR). These %different
signal sources may have %very
different frequencies. For instance, %dialysis is performed
%three times a week, blood test is biweekly, while CTR is only evaluated monthly.
blood tests and CTR are often evaluated less frequently than dialysis. Different sources may not be aligned in time and what makes things worse is that some sources may be irregularly sampled, %and be contaminated by %noises and %negligence.
%bias.
%neglected items. \scream{Previous sentence is not clear.}\yw{modified} \iffalse{Despite such discrepancies, different signals are indeed complementary to reflect a patient's %multifaceted
%physical conditions, and thus integral to any of the diagnostic analysis. }\fi
and missing entries may present. 
Despite such discrepancies, different signals give complementary views on a patient's physical condition, and therefore are all important to the diagnostic analysis.
% \scream{Perhaps reword to:  }
However, simply combining the signals will induce highly sparse MTS data.
Similar scenarios are also found in other domains: In finance, time series from financial news, stock markets, and investment banks are collected at asynchronous time steps, but are correlated strongly \cite{binkowski2018autoregressive}. In large-scale complex 
monitoring systems, sensors of multiple sub-components may have different running environments, thus continuously emitting asynchronous time series that may still be related \cite{safari2014multirate}.

%In spite of the prevalence, collectively analyzing MTS from multiple sources remains challenging due to the aforementioned high sparsity that may present 
%as a result of
%when signals are combined. 
The sparsity of MTS signals when integrated from heterogeneous sources presents several challenges.
In particular, it complicates temporal dependencies and prevents popular models, such as recurrent neural networks (RNNs), from being directly used. The most common way to handle sparsity is to first impute missing values, and then make predictions on the imputed MTS. However, as discussed in \cite{che2018recurrent}, this two-step approach fails to account for the relationship between missing patterns and predictive tasks, %thus easily 
leading to sub-optimal results when the sparsity is severe. 

Recently, some end-to-end models have been proposed. One approach is to consider missing time steps as intervals, and design RNNs with continuous dynamics via functional decays between observed time steps \cite{cao2018brits,rubanova2019latent}. %Whereas, these methods typically ignore entire vectors at some time steps, and cannot handle the non-uniform missing patterns in different dimensions.
Another approach is to parameterize all missed entries and jointly train the parameters with predictive models, so that the missing patterns are learned to fit downstream tasks \cite{che2018recurrent,shukla2019interpolation,tang2020joint}. However, these methods have the drawback that MTS samples are assessed individually. Latent relational structures that are shared by different MTS samples are seldom explored for robust modeling.% \scream{I didn't understand the previous two sentences, reworded.}
%\yw{\cite{tang2020joint} uses memory module which uses the correlations between multiple samples. Should we talk about the difference between ours and that work? I think the difference includes: 1) \cite{tang2020joint} did not explicitly learn the clustering structures and \cite{tang2020joint} did not capture the dynamics of the memory module, which is what we did. So I think our model can provide more interpretability; 2) our framework is more flexible since we can incorporate continuous time intervals; 3) \cite{tang2020joint} did not use generative model, therefore having worse performance.}

In many applications, MTS's are not independent, but are related by hidden %clustering
structures. Fig. \ref{fig.intro} shows an example of two dialysis patients. Throughout the course of treatments, each patient may experience different latent states, such as kidney disorder and anemia, which are externalized by %the recorded data,
time series, %({\em i.e.}, vectors below states),
such as glucose, albumin, and platelet levels. If two patients have similar pathological conditions, some of their data may be generated from similar state patterns, and could form clustering structures. %The complementary information in a cluster can be leveraged by learning effective states.
Thus, inferring latent states and
modeling their dynamics %modeling the dynamics of latent states, instead of isolated MTS,
are promising for leveraging the complementary information in clusters, which can %enhancing the robustness to sparsity. 
alleviate the issue of sparsity. This idea is not limited to medical domain. For example, in meteorological domain, nearby observing stations that monitor climate conditions may experience similar weathers ({\em i.e.}, latent states), % at different time, 
which govern the generation of metrics, such as temperature and precipitation, over time. Although promising, inferring the latent clustering structures while modeling the dynamics underlying sparse MTS data is a challenging problem.

To address this problem,  we propose a novel %generative model \ourmethod, based on a newly designed \underline{D}eep \underline{D}ynamic \underline{G}aussian \underline{M}ixture distribution. %Our goal is to systematically capture the latent dynamic structures governing the temporal dependencies present in sparse MTS samples, whereby performing robust MTS forecasting.
\underline{D}ynamic \underline{G}aussian \underline{M}ixture based \underline{D}eep \underline{G}enerative \underline{M}odel (\ourmethod). 
\ourmethod\ has a state space model under a non-linear transition-emission framework. For each MTS, it models the transition of latent cluster variables, instead of isolated feature representations, 
%for achieving optimal robustness, %The transition of latent clusters follows deep Markov processes, %\yw{not really Markov process. Other related works directly say that the transition is parameterized by the recurrent neural network },
%where all distributions are parameterized by neural networks. 
where all transition distributions are parameterized by neural networks.  %\scream{Took out "for achieving optimal robustness" ... didn't seem to be the right place for the comment.}
\ourmethod\ is characterized by its emission step, where a dynamic Gaussian mixture distribution is proposed to capture the dynamics of clustering structures. For inductive analysis, we resort to variational inferences, and develop structured inference networks %simultaneously learns an inference network and a generative model by %parameterized by neural networks
to approximate posterior distributions. To ensure reliable inferences, we also adopt the paradigm of parametric pre-imputation, %which is designed to estimate missing values by (1) a trainable temporal intensity function for encoding temporal dependencies, and (2) a set of correlation parameters for capturing multi-variable relationships.
%All parameters are trained jointly, and
and link a pre-imputation layer ahead of the inference networks. The entire \ourmethod\ model is carefully designed to handle discrete variables and is constructed to be end-to-end trainable. %so that the missing patterns are learned to well align with the generative tasks.
Our contributions are summarized as follows:
\begin{itemize}
\item We investigate the problem of sparse MTS forecasting by modeling the latent dynamic clustering structures.%leveraging the latent dynamic structures shared by sparse MTS samples for robust modeling and forecasting.
\item We propose \ourmethod, %with %a generative network based on
%a novel dynamic Gaussian mixture based emission process, and a structured inference network that models the dynamics of cluster variables.
a novel deep generative model that leverages the transition of latent clusters and the emission from dynamic Gaussian mixture for robust forecasting.
\item We perform extensive experiments on real-life datasets to validate the %state-of-the-art performance
effectiveness of our proposed method.
\end{itemize}
% gate?
% three perspectives of relationships (1) temporal dependencies, (2) multi-dimensional correlation, and (3) latent clustering structures.










==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
